Near-Involutions, the Pillowcase Distribution, and Quadratic Differentials

In the context of A. Eskin and A. Okounkov's approach to the calculation of the volumes of the different strata of the moduli space of quadratic differentials, two objects have a prominent role. Namely, the characters of near-involutions and the pillowcase weights. For the former we give a fairly explicit formula. On the other hand, the pillowcase weights induce a distribution on the space of Young diagrams. We analyze this distribution and prove several facts, including that its limit shape corresponds to the one induced by the uniform distribution, that the probability concentrates on the set of partitions with very similar 2-quotients, and that there is no hope for a full Central Limit Theorem. This is a reformatted version of the author's Ph.D. thesis, advised by Professor Andrei Okounkov. The results will be published in a forthcoming paper.

==> expointro.tex <==
\todoreminder{Revise this part}

This chapter is an exposition of \cite{pillow}.

In Section \ref{howtocomputethevolume}, it was explained that the asymptotics of the generating function \eqref{generatingfunction} is central to the computation of the volume of the strata of the moduli space of quadratic differentials.

The first thing to notice about this generating function is that it can be interpreted as an expectation of a certain function with respect to the pillowcase distribution. Recall balanced partitions are those for which the sum in equation \eqref{balanced} vanishes. The pillowcase distribution is defined by
\[\mathbb P(\lambda)=
\left\{\begin{array}{ll}q^{|\lambda|} \w(\lambda)/Z, &  \textrm{$\lambda$ balanced,} \\
0,&\textrm{otherwise,}\end{array}
\right.\]
where $\lambda$ is any partition, $\w(\lambda)$ is the pillowcase weight, defined in equation \eqref{pillowcaseweight}, $q$ is a complex parameter with $|q|<1$, and $Z$ is a normalization constant:
\[Z=Z(\emptyset,\emptyset;q)=\sum_\lambda q^{|\lambda|}\w(\lambda).\]
If we set
\[\mathbf g_\nu(\lambda)=\frac{\mathbf f_{(\nu,2,2,\dots)}(\lambda)}{\mathbf f_{(2,2,\dots)}(\lambda)},\]
we can write
\[\frac{Z(\mu,\nu;q)}Z=\left\langle \mathbf g_\nu(\lambda) \prod_i\mathbf f_{\mu_i}(\lambda)\right\rangle_\w\]
We will see in Section \ref{shiftedsymmetricalgebra} \todoreminder{Promises promises\dots}that both the functions $\mathbf g_\nu$ and the functions $\mathbf f_{\mu_i}$ belong to the algebra $\overline \Lambda$ generated by the shifted symmetric power functions $\p_k$ and their twisted counterparts $\pbar_k$.

\todoreminder{Show that $|\mathsf w|<1$.} 




==> inclusionexclusion.tex <==
As explained in Section \ref{howtocomputethevolume}, the expectation $\langle\g_\nu\rangle_\w$ gives the volume of the stratum of the moduli space of \emph{disconnected} quadratic differentials with zeroes and poles of orders $(k_1,\dots,k_\ell)=(\nu_1-2,\nu_2-2,\dots,\nu_\ell-2)$. `Disconnected' here means that these quadratic differentials may be defined disconnected Riemann surfaces.

In order to compute the volumes of the strata of \emph{connected} quadratic differentials, we need to use the \emph{inclusion-exclusion} principle. This works as follows.  

==> intromychapter.tex <==
As in the approach of A. Eskin and A. Okounkov (see Sections \ref{howtocomputethevolume} and \ref{asymptotics}), we start by considering the generating function \eqref{generatingfunction} as an expectation
\[\left\langle\g_\nu \right\rangle_\w\]
of the functions $\f_{\mu_i}$, where
\[\f_{\eta}(\lambda)=|C_{\mu}|\frac{\chi^\lambda(\eta)}{\dim\lambda}\]
and in this case $\eta=(\mu_i,1,1,\dots,1)$, and the functions
\[\g_\nu(\lambda)=\frac{\f_{(\nu,2,2,\dots,2)}(\lambda)}{\f_{(2,2,\dots,2)}(\lambda)}\]
with respect to the probability distribution induced by the pillowcase weights, given by
\[\w(\lambda)=\left(\frac{\dim\lambda}{|\lambda|!} \right)^2\f_{(2,2\dots,2)}(\lambda)^4,\]
multiplied by $q^{|\lambda|/2}$ for a complex parameter $q$, $|q|<1$, so that 
\[\left\langle\g_\nu\right\rangle_\w=\sum_\lambda q^{|\lambda|/2}\w(\lambda)\g_\nu(\lambda).\]
In this chapter, we will prove that this distribution induces a \emph{limit shape}, that is, that there is a curve $\Omega$ such that, as $|\lambda|\to\infty$, the $\w$-probability for the edge of an appropriately rescaled, arbitrary Young diagram to be close to $\Omega $ tends to 1. The limit shape coincides with the one for the uniform partitions; see Section \ref{limitshapeuniform}.

An immediate consequence is that we will be able to compute the values of the expectations $\langle\p_k\rangle_\w$. We will use this result again to compute the expectations $\langle \g_\nu\rangle_\w$. These calculations are finalized in Chapter \eqref{conclusionschapter}.

The proof of the central limit theorem consists of two steps. The first one is writing $\w$ as a quotient of hook lengths. The second is an argument similar to the one used by S. Kerov and A. Vershik \cite{vershikkerov1985} to obtain the limit shape in the case of the Plancherel distribution. 

==> pclimitshape.tex <==
In this section, we will compute, using the tools developed by A. Eskin and A. Okounkov \cite{pillow}, the limit shape of the pillowcase distribution, which coincides with the limit shape for the uniform distribution.

Let $F(\lambda)$ denote the Frobenius coordinates $\{\lambda_i-i+\frac12\}_{i\geq0}\subseteq \Z+\frac12$ of a partition $\lambda=(\lambda_1,\lambda_2, \dots,\lambda_n)$.  We want to calculate the probability
\[p(u)=\mathbb P_\w(u\in F(\lambda))=\frac{\sum_{F(\lambda)\ni u}\w(\lambda) q^{|\lambda|/2} }{\sum_{\textrm{all $\lambda$}}\w(\lambda) q^{|\lambda|/2}}, \quad u \in \Z+\frac12.\]
The probability $p(u)$ gives the expectation that the maya diagram will have a black pebble at the point $u$ (see Section \ref{fock}); the complementary probability $1-p(u)$ corresponds to having a white pebble at $u$. This in turn means that we will have slope $1$ with probability $p(u)$ and slope $-1$ with probability $1-p(u)$. Taking the limit, as $|\lambda|\to\infty$, we see that the limit shape $\Phi(u)$ (in the coordinates that have been rotated $135^\circ$, as in Section \ref{fock}) should satisfy
\[ \Phi'(u)=\lim_{q\to+\infty}2p\left(\frac{u}{1-q}\right)-1,\]
because, as we shall see, $\langle|\lambda|\rangle_\w=(1-q)^2$. \todoreminder{Prove that.}

We define the theta function $\vartheta$ as in Section \ref{jacobithetas}:
\[\vartheta(x)=(q^{1/2}-q^{-1/2})\prod_{i=1}^\infty\frac{(1-q^ix)(1-q^i/x)}{(1-q^i)^2}.\]
The notation $[m]f(x,y)$ means: ``expand $f$ as a series in the variables involved in the monomial $m$ and take the coefficient of $m$.''

\begin{prop}\label{prop:closedformula}
We have:
\begin{equation}\label{eq:closedformula}
p(u)=[x^uy^0]\frac{1}{\vartheta(x)}\sqrt{
\frac{\vartheta(-y)\vartheta(xy)}{\vartheta(y)\vartheta(-xy)}}.
\end{equation}
and
\begin{equation}\label{eq:sumofweights}
\sum_{\textrm{all $\lambda$}}q^{|\lambda|/2}\w(\lambda)= \prod_i(1-q^{2i})^{-1/2},
\end{equation}
\end{prop}
\begin{rmk}
It is important to remark that the expansion with respect to $x$ and $y$ should be taken in the domain
\[|y/q|>|xy|>|y|>1,\]
because that is where the generating functions above converge.
Observe that $p$ is essentially a coefficient of the 1-point function in \cite{pillow}.
\end{rmk}
\begin{proof}
We first explain how to compute the numerator of $p(u)$, namely, $\sum_{F(\lambda)\ni u}\w(\lambda)q^{|\lambda|/2}$. It will be clear that the denominator can be calculated similarly. In the context of the Fock space representation $\Lambda^{\frac{\infty}2}_0$ (see Section \ref{fock} for definitions and notations), we consider the vertex operator
\[\pcop =\exp\left(\sum_{n>0}\frac{\alpha_{-2n-1}}{2n+1}\right) \exp\left(-\sum_{n>0}\frac{\alpha_{2n+1}}{2n+1}\right).\]
The form of $\pcop$ was probably guessed using the tools developed by A. Borodin, A. Okounkov and G. Olshanski \cite{borodinokounkovolshanski}.
In the paper \cite{pillow}, $\pcop$ is called the \emph{pillowcase operator} because we have
\begin{thm}[\protect{\cite[Theorem 4]{pillow}}]
The diagonal matrix elements of $\pcop$ are as follows:
\[\langle\pcop \,v_\lambda,v_\lambda\rangle=\left\{\begin{array}{ll}
\w(\lambda), &\textrm{if $\lambda$ is balanced,} \\
0, & \textrm{otherwise.}
\end{array}\right.\]
\end{thm}

We omit the proof. Continuing now with the proof of Proposition \ref{prop:closedformula}, set
\[\psi(x)=\sum_{k\in \Z+\frac12}x^k\psi_k\quad\textrm{and}\quad
\psi^*(x)=\sum_{k\in \Z+\frac12}x^{-k}\psi_k^*,\]
and let $H$ be the energy operator, given by
\[Hv_\lambda=|\lambda|v_\lambda.\]
Then
\begin{equation}\label{eq:intermediatestep}
\sum_{k\in \Z+\frac12} x^k\sum_{F(\lambda)\ni u} q^{|\lambda|/2} \w(\lambda)=[y^0]\trace q^{H/2}\pcop \,\psi(xy)\psi^*(y).
\end{equation}
This works because
\[\psi_k\,\psi^*_k\, v_\lambda=\left\{\begin{array}{ll}v_\lambda,&x\in F(\lambda) \\
0, & \textrm{otherwise,}\end{array}\right.\]
and the operation of taking the coefficient of $y^0$ eliminates all other combinations of the form $\psi_k\psi^*_l$ with $k\neq l$.
Using the identity \cite[Theorem 14.10]{kac},
\begin{multline*}
\psi(xy)\psi^*(y)=\frac 1{x^{1/2}-x^{-1/2}}
\exp\!\left(\sum_{n\geq 1}\frac{(xy)^n-y^n}n\alpha_{-n}\right) \exp\!\left(\sum_{n\geq 1}\frac{y^{-n}-(xy)^{-n}}n\alpha_n\right),
\end{multline*}
it is straightforward, using also the fact that $[\alpha_n,\alpha_m]=0$ if $nm<0$, to see that we are looking for the trace
\[\trace\frac{q^{H/2}}{x^{1/2}-x^{-1/2}}\exp\!\left(\sum_{n\geq 1} \frac{(xy)^n-y^n+\deltaodd}n\alpha_{-n}\right)\exp \!\left(\sum_{n\geq1}\frac{y^{-n}-(xy)^{-n}-\deltaodd}n\alpha_n\right).\]
Observe that this operator factors through the decomposition
\[\Lambda^{\frac\infty2}_0\cong \bigotimes_{n=1}^\infty\bigoplus_{k=0}^\infty \C\alpha_{-n}^k v_\emptyset,\]
and in each of these factors the trace can be computed using the identity
\[\left.\trace q^{H/2}e^{A\alpha_{-n}}e^{B_{\alpha_n}}\right|_{\bigoplus_{k=0}^\infty \C \alpha^k_{-n}v_\emptyset} = \frac1{1-q^n}\exp\!\left(\frac{nAB\,q^n}{1-q^n}\right).\]
that can be verified directly by examining the series expansions of both sides.
The trace above becomes
\begin{multline*}
\frac1{x^{1/2}-x^{-1/2}}\prod_{n=1}^\infty \frac{1}{1-q^n}\times\\ \exp\!\left(
\frac{nq^n}{n^2(1-q^n)}((xy)^n-y^n+\deltaodd)(y^{-n}-(xy)^{-n}-\deltaodd)\right)\\
=\frac{\prod_{n=1}^\infty (1-q^n)^{-1}}{x^{1/2}-x^{-1/2}}\exp\left(\sum_n\frac{q^n}{n(1-q^n)}\left(
x^n+x^{-n}-2\right)
\right)\times \\
\exp\left(
\sum_{\textrm{$n$ odd}} \frac{q^n}{n(1-q^n)}\left(y^n+y^{-n}-(xy)^{-n}-(xy)^{n}\right)
\right)
\end{multline*}
Expanding the series of the denominator inside the exponent, $1-q^n$, exchanging the order of summation, and the identity
\[\log (1-x)=-\sum_{n=1}^\infty\frac {x^n}n,\quad |x|<1,\]
lead to
\begin{multline*}
\frac{\prod_{n=1}^\infty (1-q^n)^{-1}}{x^{1/2}-x^{-1/2}}\times \\
\exp\sum_{i=1}^\infty\left(-\log(1-q^ix)-\log(1-q^i/x)+2\log(1-q^i)\right)\times\\
\exp\frac12\sum_{i=1}^\infty\left(\log(1+q^iy)+\log(1-q^i/y)-\log(1-q^iy)-\log(1-q^i/y)+\right.\\
\log(1-q^ixy)+\log(1-q^i/(xy))-\log(1+q^ixy)-\log(1+q^i/(xy)+\\
\left.\log(1-q^i)-\log(1+q^i))\right)
\end{multline*}
The above is easily seen to simplify to
\begin{equation}\label{eq:numerator}
\frac{\prod_i(1-q^{2i})^{-1/2}}{\vartheta(x)}[y^0]\sqrt{
\frac{\vartheta(-y)\vartheta(xy)}{\vartheta(y)\vartheta(-xy)}}.
\end{equation}
This is the right hand side of equation \eqref{eq:intermediatestep}. Taking the coefficient of $x^u$, we find the numerator of $p(x)$.

The denominator of $p(u)$ is similarly seen to be equal to
\[[y^0]\trace q^{H/2}\,\psi(xy)\psi^*(y),\]
and hence to satisfy
\eqref{eq:sumofweights},
so $p(x)$ is indeed as in equation \eqref{eq:closedformula}.
\end{proof}

With that settled, we now want to see that the following is true:
\begin{prop}
\[\lim_{q\to+\infty}p\!\left(\frac{u}{1-q}\right)=\frac1{1+e^u}.\]
\todoreminder{Fix this.}
\end{prop}
\begin{proof}

We first perform the operation of obtaining the coefficient of $y^0$ in \eqref{eq:closedformula}. Let $q=e^{2\pi i \tau}$, $x=e^{2\pi i z}$, $y=e^{2\pi i w}$. We want to take the integral
\begin{equation}\label{eq:limitshapeintegral}
[y^0]\sqrt{\frac{\vartheta(-y)\vartheta(xy)}{\vartheta(y)\vartheta(-xy)}}=
\frac1{2\pi i} \oint_{|y|=1}\sqrt{\frac{\vartheta(-y)\vartheta(xy)}{\vartheta(y)\vartheta(-xy)}}\frac{dy}y=
\int_{0}^{1}\sqrt{ \frac{ \vartheta(w+\frac12)\vartheta(z+w)}
{\vartheta(w)\vartheta(z+w+\frac12)}} \,dw.
\end{equation}
Since
\[\vartheta(z,\tau)=-i\eta^{-3}(\tau)\vartheta_{11}(z,\tau)\]
(see Section \ref{jacobithetas}), the quotient inside the square root is
\[\frac{\vartheta_{11}(w+\frac12)\vartheta_{11}(w+z)} {\vartheta_{11}(w)\vartheta_{11}(w+z+\frac12)}.\]
Using the identities between the different Jacobi theta functions given in Section \ref{jacobithetas}, we see that
\[\vartheta_{11}(w+\frac12)=-\vartheta_{10}(w),\]
so the quotient above equals
\[\frac{\vartheta_{10}(w)\vartheta_{11}(w+z)}{\vartheta_{11}(w)\vartheta_{10}(w+z)}.\]
Applying the modular transformation $\tau\mapsto -1/\tau$, this becomes
\[\frac{\vartheta_{01}\!\left(\frac w\tau,-\frac1\tau\right) \vartheta_{11}\!\left(\frac{w+z}\tau,-\frac1\tau\right)}
{\vartheta_{11}\!\left(\frac w\tau,-\frac1\tau\right) \vartheta_{01}\!\left(\frac{w+z}\tau,-\frac1\tau\right)},\]
---all other terms cancel out--- and then we can look at the Fourier expansions of the functions involved to derive the asymptotics as $\tau\to0$. First,
\begin{align*}
\vartheta_{01}\!\left(\frac w\tau,-\frac1\tau\right)=
\sum_{n\in\Z}(-1)^n\exp-\frac{\pi i}\tau\left((n-w)^2-w^2\right)\approx
\pm\exp-\frac{\pi i}\tau\left(\{w\}^2-w^2\right),
\end{align*}
where $\{w\}$ stands for the difference between $w$ and the integer that is closest to it.
Similarly,
\begin{align}
\vartheta_{11}\!\left(\frac w\tau,-\frac1\tau\right)&=
\sum_{n\in \Z}(-1)^{n+\frac12} \exp -\frac{\pi i}\tau\left(\left(n+\frac12-w\right)^2-w^2\right) \notag\\
&\approx
\pm i\exp-\frac{\pi i}\tau\left(\left\{w-\frac12\right\}^2-w^2\right).
\label{eq:thetaapproximation}
\end{align}
Note that these are very good approximations because the neglected terms are exponentially smaller in $1/\tau$.
Taking these approximations, the integral \eqref{eq:limitshapeintegral} equals
\[e^{i\pi z/2\tau}\left(\frac{i\tau}\pi  \left(1-e^{i\pi z/\tau}\right)
\pm (1-z)\right).\]
Call this expression $g(z,\tau)$.

Now we want to find the coefficient of $x^u$ in \eqref{eq:closedformula}. This entails taking the integral
\[\frac{1}{2\pi i}\oint_{|x|=1} \frac{g(z,\tau)}{\vartheta(x,q)}\frac{dx}{x^{u+1}}= \int_0^1 \frac{g(z,\tau)}{\vartheta(z,\tau)}\frac{dz}{e^{2\pi i z u}}.\]
Neglecting a factor that depends on only on $\tau$, we can use again the approximation \eqref{eq:thetaapproximation} for the $\vartheta$ factor in the denominator. We get

\end{proof}


==> shiftedsymmetric.tex <==
Denote the algebra of symmetric functions by $\Lambda$. This is algebraically generated by the symmetric power functions
\[p_k(x_1,x_2,\dots)=\sum_{i=1}^\infty x_i^k;\]
see Section \ref{symmetricfunctions}.

Let $\Lambdastar$ be the algebra of the shifted-symmetric functions, generated by the shifted-symmetric power functions $\p_k$ with coefficients in the field of the rational numbers $\Q$, and let $\Lambdabar$ be the extension of $\Lambda$ that also contains the $\Z/2\Z$-twisted shifted-symmetric power functions $\pbar_k$. For convenience, we recall the definitions of these functions:
\begin{align*}
\p_k(\lambda)&=\sum_i[(\lambda_i-i+\frac12)^k-(-i+\frac12)^k]+c_k,\\
\pbar_k(\lambda)&=\sum_i[(-1)^{\lambda_i-i+1}(\lambda_i-i+\frac12)
-(-1)^{-i+1}(-i+\frac12)]+c_k'.
\end{align*}
The constants $c_k$ and $c_k'$ are chosen so that equation \eqref{constantsforps} is satisfied.

In this section we prove the following two lemmas:

\begin{lem}[\protect{\cite{kerovolshanski,okounkovolshanski}}]\label{lemmafs}
The functions $\mathbf f_\mu$ are polynomials in the shifted-symmetric functions $\p_k$, i.e., $\mathbf f_\mu \in \Lambdastar\subset \Lambdabar$.
\end{lem}

\begin{lem}[\protect{\cite{pillow}}]\label{lemmags}
The functions $\mathbf g_\nu$ are polynomials in the functions $\p_k$ and $\pbar_k$, i.e., $\mathbf g_\nu\in \Lambdabar$.
\end{lem}

\begin{proof}[Proof of Lemma \ref{lemmafs}]

\end{proof}
\begin{proof}[Proof of Lemma \ref{lemmags}]

\end{proof}
